Pricing Energy Storage in Real-time Market

The problem of pricing utility-scale energy storage resources (ESRs) in the real-time electricity market is considered. Under a rolling-window dispatch model where the operator centrally dispatches generation and consumption under forecasting uncertainty, it is shown that almost all uniform pricing schemes, including the standard locational marginal pricing (LMP), result in lost opportunity costs that require out-of-the-market settlements. It is also shown that such settlements give rise to disincentives for generating firms and storage participants to bid truthfully, even when these market participants are rational price-takers in a competitive market. Temporal locational marginal pricing (TLMP) is proposed for ESRs as a generalization of LMP to an in-market discriminative form. TLMP is a sum of the system-wide energy price, LMP, and the individual state-of-charge price. It is shown that, under arbitrary forecasting errors, the rolling-window implementation of TLMP eliminates the lost opportunity costs and provides incentives to price-taking firms to bid truthfully with their marginal costs. Numerical examples show insights into the effects of uniform and non-uniform pricing mechanisms on dispatch following and truthful bidding incentives.

==> PricetakerBidIncentiveV2.tex <==


\subsection{{Sufficient Condition to check untruthfully bidding incentives under rolling-window uniform pricing for generators}}  
\tcr{we can eliminate all $i$ for simplicity in this version}\\
Let $\qbf_i(\cdot) = (q_{i1}(\cdot), \cdots, q_{iT}(\cdot))$ be the true marginal cost of generation $i$  over $T$ intervals.  Let $\fbf_i(\cdot | \theta_i) = (f_{it}(\cdot |\theta_{it}))$ be the generator's bid-in cost  (supply) curve  parameterized by  $\thetabf_i = (\theta_{it})$.  Assume that, at $\thetabf_i=\thetabf^*_i$,   $\fbf_i(\cdot | \theta^*_i)= \qbf_i(\cdot)$.   

It's already show in \cite{Guo&Chen&Tong:20arxiv} that there does not exist a uniform pricing scheme under which all generators have zero LOC. So the total profit of a price taker generator $i$ is given by
\beq \label{eq:Pi_i}
\begin{array}{l}
 \Pi_i(\thetabf_i) = \pibf^{\T} \gbf^{\RED}_i(\thetabf_i) - \sum_{t=1}^T q_{it}(g^{\RED}_{it}(\theta_{it}))\\
+\max_{\gbf_i}\pibf^{\T} \gbf_{i} - \sum_{t=1}^T f_{it}(g_{it}|\theta_{it})\\
- \pibf^{\T} \gbf^{\RED}_i(\thetabf_i) + \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}),
\end{array}
\eeq
where, under the price-taker assumption,  the uniform clearing price $\pibf$  is not a function of $\thetabf_i$. $\{g^{\RED}_{it}(\thetabf_{i})\}$ is the rolling-window economic dispatch over the entire scheduling horizon $\Hc$ under a uniform clearing price $\{\pi_t\}$. The first row of (\ref{eq:Pi_i}) is the generation surplus and the lost opportunity cost (LOC) under the bid-in cost curve $\fbf_i(\cdot | \theta_i) = (f_{it}(\cdot |\theta_{it}))$ is represented by the second and third row.

%Let $f_{it}(\cdot|\theta_{it})=\frac{1}{2}\theta_{it}g_{it}^2$. First to solve the optimal value of 
Specifically, The second row of (\ref{eq:Pi_i}) follows optimization below:
\beq \label{eq:LOC}
\begin{array}{rll}
&\underset{\gbf_i}{\rm minimize} &  \sum_{t=1}^T f_{it}(g_{it}|\theta_{it})-\pibf^{\T}\gbf_{i}\\
 & {\rm subject~to}&
 (\underline{\etabf}_{i},\bar{\etabf}_{i}):~~ -\underline{\rbf}_i\leq \Abf\gbf_i \leq \bar{\rbf}_i, \\
 & & (\underline{\zetabf}_{i},\bar{\zetabf}_{i}):~~   {\bf 0}\leq \gbf_i \leq\bar{\gbf}_{i}.
\end{array} \hfill
\eeq
By the KKT condition, the optimal solution of the above must satisfy
\beq \label{eq:LOCKKT}
\nabla_{\gbf_{i}} f_i(\gbf^*_{i}|\thetabf_{i})-\pibf +\Abf^{\intercal}\Delta\etabf^*_{i} + \Delta\zetabf^*_{i} ={\bf 0},
\eeq
where $\Delta\etabf^*_{i}=\bar{\etabf}^*_{i} - \underline{\etabf}^*_{i}$ and $\Delta\zetabf^*_{i}=\bar{\zetabf}^*_{i} - \underline{\zetabf}^*_{i}$. 


So we can rewrite \eqref{eq:Pi_i} into 
\beq \label{eq:Pi_i2}
\begin{array}{l}
 \Pi_i(\thetabf_i) = \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\thetabf_{i})|\theta_{it})- \sum_{t=1}^T q_{it}(g^{\RED}_{it}(\thetabf_{i}))\\
+\pibf^{\T}\gbf^*_{i}-\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it}),
\end{array}
\eeq


The following theorem establishes that $\thetabf=\thetabf^*$  is not the maximizer of $\Pi_i(\thetabf_i)$ defined in (\ref{eq:Pi_i}), \ie bidding at the true cost is not the optimal. 


\begin{theorem}[{Untruthful bidding incentives under rolling-window uniform pricing}] \label{thm:UntruBidUniformPricingLOC}
Let $\{g_{it}^{\RED}(\thetabf_{i})\}$ be the rolling-window economic dispatch over the entire scheduling horizon $\Hc$ when bid-in cost parameter is $\thetabf_i$. There does not exist a uniform pricing scheme under which a price taker generators $i$ will bid truthfully over $\Hc$  such that
\ben

\item  generators $i$ have $\frac{\partial}{\partial \theta_{it} \partial g_{it}}f_{it} > 0$ for bid-in cost (supply) curve. 
\item  generators $i$ has nonzero LOC under rolling-window dispatch,$\{g_{it}^{\RED}(\thetabf_{i}^*)\}$, and $\forall t, g_{it^*}^{\RED}(\thetabf^*_{i}) \in \{0,\bar{g}_i\}$ or the ramping constraints from $t^*-1$ to $t^*$ or from $t^*$ to $t^*+1$ is binding. 
\item  $\forall t, g_{it^*}^{*}(\thetabf^*_{i}) \in \{0,\bar{g}_i\}$ or the ramping constraints from $t^*-1$ to $t^*$ or from $t^*$ to $t^*+1$ is binding. 



 \een
\end{theorem}

\textit{Proof:} Because generator $i$ has nonzero LOC, we have $\gbf^*_{i} \neq \gbf^{\RED}_{i}$.
From conditions  3) of Theorem~\ref{thm:UntruBidUniformPricingLOC}, we know $\bar{\etabf}^*_{i}\underline{\etabf}^*_{i}\bar{\zetabf}^*_{i}\underline{\zetabf}^*_{i}\neq \mathbf{0}$ 
%Let $\Delta\eta^*_{it}\neq 0$
 We argue that any infinitesimal change in $f_{it}(\cdot|\theta_{it})$ will not change the optimal solution $\gbf^*_{it}$, \ie   $\frac{\partial}{\partial \theta_{it}} g^{\mbox{\tiny *}}_{it}(\thetabf_i)=0$. Specifically, suppose that an infinitesimal change of $\theta_{it}^*$ causes a change  $f_{it}(g_{it}^{*}|\theta_{it}) = f_{it}(g_{it}^{*}|\theta_{it})+ \epsilon$.  By the continuity of $f_{it}$ with respect to $\theta_{it}$ and  (\ref{eq:LOCKKT}),  we can always reduce  $\Delta\eta^*_{i(t-1)}-\Delta\eta^*_{it} + \Delta\zeta^*_{it}$ by  $\epsilon$ so that the KKT condition \eqref{eq:LOCKKT} is still satisfied. Moreover, as long as $\epsilon$ is small enough, all other inequalities in KKT conditions will also hold. Similarly, it can be proved that $\frac{\partial}{\partial \theta_{it}} g^{\mbox{\tiny \RED}}_{it}(\thetabf_i)=0$

%This can also be observed from  \eqref{eq:LOCKKTDerTheta}.
%So we have $\gbf^*_{i}=\nabla f_i^{-1}(\pibf -\Abf^{\intercal}\Delta\etabf^*(\theta_{it}) - \Delta\zetabf^*(\theta_{it}))$. And the optimal value is $\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})-\pibf^{\T}\gbf^*_{i}$.

% Take derivative over $\thetabf_{i}$ on both sides of (\ref{eq:LOCKKT}). We have
% \beq \label{eq:LOCKKTDerTheta}
% \nabla_{\thetabf_{i}}\nabla_{\gbf^*_{i}} f_i(\gbf^*_{i}|\thetabf_{i})+\nabla_{\thetabf_{i}} \gbf^*_{i}\nabla^2_{\gbf^*_{i}} f_i(\gbf^*_{i}|\thetabf_{i}) +\nabla_{\thetabf_{i}}(\Abf^{\intercal}\Delta\etabf^*_{i}) + \nabla_{\thetabf_{i}}(\Delta\zetabf^*_{i}) ={\bf 0},
% \eeq

And the derivative of \eqref{eq:Pi_i2} over $\theta_{it}$ can be simplified as
\beq \label{eq:Pi_i2Derivative}
\begin{array}{l}
 \frac{\partial}{\partial \theta_{it}} \Pi_i(\thetabf_i) = \frac{\partial}{\partial \theta_{it}} f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it})-\frac{\partial}{\partial \theta_{it}} f_{it}(g^*_{it} |\theta_{it}),
\end{array}
\eeq

We already know $\gbf^*_{i} \neq \gbf^{\RED}_{i}$ and $\frac{\partial}{\partial \theta_{it} \partial g_{it}}f_{it} > 0$ . So  $\nabla_{\tiny \thetabf_{i}} \Pi_i(\thetabf_i)  \neq  \mathbf{0}$.
To make more profits, a generator will increase $\theta_{it}$ at $t$ when $g^*_{it} < g^{\RED}_{it}$, and decrease $\theta_{it}$ at $t$ when $g^*_{it} > g^{\RED}_{it}$.


% From \eqref{eq:LOC}, we also know that $ \sum_{t=1}^T f_{it}(g^*_{it}|\theta_{it})-\pibf^{\T}\gbf^*_{i} \le  \sum_{t=1}^T f_{it}(g^{\RED}_{it}|\theta_{it})-\pibf^{\T}\gbf^{\RED}_{i}$

% to show $\exists \pibf, s.t. $

% \tcr{Further complete}Make asumptions $g^{\RED}$ and $g^*$ both unchange when $\theta$ change. And linear cost function.Then
% \beq \label{eq:toycase}
% \begin{array}{l}
% & \Pi_i(\thetabf_i) = \sum_{t=1}^T f_{it}(g^{\RED}_{it}|\theta_{it})-\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})
% &=\theta_{i}\sum_{t=1}^T(g^{\RED}_{it}-g^*_{it}),\\
% \end{array}
% \eeq
% As $\sum_{t=1}^T(g^{\RED}_{it}-g^*_{it})>0$,$\theta_{i}$ is used for all intervals. $\frac{\partial }{\partial \theta_{i}}\Pi_i(\thetabf_i)=\sum_{t=1}^T(g^{\RED}_{it}-g^*_{it}) >0$.

% \tcr{Further complete}Make asumptions $g^{\RED}$ and $g^*$ both unchange when $\theta$ change and $g^{\RED} 
% \geq g^*$. And $\frac{\partial^2 f_{it}}{\partial \theta_{it} \partial g_{it}}>0$. Then we need to compare only this part $\Pi_i(\thetabf_i) = \sum_{t=1}^T f_{it}(g^{\RED}_{it}|\theta_{it})-\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})$.
% \beq \label{eq:Pi_i2Derivative}
% \begin{array}{l}
% & \frac{\partial }{\partial \theta_{ik}}\Pi_i(\thetabf_i) =\sum_{t=1}^T (\frac{\partial }{\partial \theta_{it}}f_{it}(g^{\RED}_{it}|\theta_{it})-\frac{\partial }{\partial \theta_{it}}f_{it}(g^{*}_{it}|\theta_{it})),
% \end{array}
% \eeq

% If the generator bids truthfully with its marginal cost of generation,  $\thetabf=\thetabf^*$ and $f_t(\gbf^{\RED}|\theta_t)= q_t(\gbf^{\RED})$, Eq. \eqref{eq:dsdq} becomes
% \beq
% \frac{\partial}{\partial \theta_k} \Pi (\thetabf^*)= \sum_{t} \frac{\partial}{\partial \theta_k^*} g^{\mbox{\tiny R-ED}}_t(\thetabf)\Delta\rho^*_t = 0, \label{eq:dsdq4}
% \eeq
% % The KKT condition gives
% % \bea \label{eq:KKT}
% % \nabla f_i(\gbf_i^*) - \lambdabf^* + \Abf^{\intercal}\Delta\mubf_i^* + \Delta\rhobf_i^* = {\bf 0}
% % \eea
% % where $\Delta\mubf_i^*=\bar{\mubf}^*_i - \underline{\mubf}^*_i$ and $\Delta\rhobf_i^*=\bar{\rhobf}^*_i - \underline{\rhobf}^*_i$.



% \tcr{Try lower bound analysis, but this may be incorrect}
% We have $\max_{g_{it}}\pibf^{\T} g_{it} - \sum_{t=1}^T f_{it}(g_{it}|\theta_{it}) \geq 0$. Besides, note that $\forall t, g^{\RED}_{it}(\theta_{it})\le \bar{g}_i$, and the bid-in cost (supply) curve is increasing, so $q_{it}(g^{\RED}_{it}(\theta_{it})) \le q_{it}(\bar{g}_i)$, so we have
% \beq 
% \begin{array}{lcl}
% &\Pi_i(\thetabf_i) &\geq - \sum_{t=1}^T q_{it}(g^{\RED}_{it}(\theta_{it})) + \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}) \\
% &&\geq \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}) - \sum_{t=1}^T q_{it}(\bar{g}_i)
% \end{array}
% \eeq

% We know that $\sum_{t=1}^T q_{it}(\bar{g}_i)$ is a finite constant, and $\lim_{\theta_i \rightarrow +\infty}  f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}) \rightarrow +\infty$. So the lower bound

% \tcr{not ok, as max part will influence}Make asumptions like linear cost curve, to have max optimal value is 0 even when $\theta$ change a little bit. \tcr{ attention: $\frac{\partial f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it})}{\partial \theta_{ik}}\neq \frac{\partial}{\partial \theta_{ik}} g^{\RED}_{it}\thetabf_{i}) (\frac{\partial}{\partial g}f_{it}(g^{\RED}_{it}|\theta_{it})$, so below is wrong and toy case is an example.}
% \beq \label{eq:Pi_i2Derivative}
% \begin{array}{l}
% & \frac{\partial \Pi_i(\thetabf_i)}{\partial \theta_{ik}} =\sum_{t=1}^T \frac{\partial}{\partial \theta_{ik}} g^{\RED}_{it}(\thetabf_{i}) (\frac{\partial}{\partial g}f_{it}(g^{\RED}_{it}|\theta_{it})- \frac{\partial}{\partial g} q_{it}(g^{\RED}_{it})),
% \end{array}
% \eeq



==> PropertiesTLMPStorage.tex <==
%\subsection{Surplus of ISO under TLMP (for storages)}

All properties below are parallel to those in in \cite{Guo&Chen&Tong:20arxiv} \cite{Chen&Guo&Tong:20arxiv}. We showed that the properties TLMP have for ramping will also hold at TLMP for storages.

In one shot optimization, surplus of ISO under TLMP (for storages) will always be nonnegative.
% $MS=consumer payment - payment to generators - payment to storages\\
% =\sum_{t=1}^{T}((\bar{E}-E^0)\bar{\delta_{t}^*})+\sum_{t=1}^{T}((E^0-\underline{E})\underline{\delta_{t}^*})$\\
And we know initial SOC has the relationship $\underline{E} \le E^0 \le \bar{E}$.

\begin{proposition}[One-shot TLMP as a strong equilibrium price for storage] \label{prop:TLMP1MS}  When there is no forecasting error, \ie $\hat{\dbf}=\dbf$, the one-shot multi-interval economic dispatch policy $\Gc^{{}^{\tiny\rm ED}}$  and the TLMP policy $\Pc^{{}^{\tiny\rm TLMP}}$ form a strong equilibrium, thus there is no incentive for any storage to deviate from the economic dispatch signal.

In addition, the one-shot TLMP guarantees revenue adequacy for the operator with total merchandising surplus equal to the SOC charge and ramping charge:
 \beq\label{eq:MS}
 \begin{array}{lcl}
 \mbox{\rm MS} &:=&\sum_t \pi^{\TLMP}_{0t}d_t-\sum_{i>0,t}( \pi^{G}_{it}g^{G}_{it}+\pi^{D}_{it}g^{D}_{it}-\pi^{C}_{it}g^{C}_{it}) \nn\\
 &=& \sum_{t=1}^{T}((\bar{E}-E^0)\bar{\delta_{t}^*})+\sum_{t=1}^{T}((E^0-\underline{E})\underline{\delta_{t}^*})\\
 &&+\sum_{i,t} (\bar{\mu}^*_{it}\bar{r}_i + \underline{\mu}^*_{it}\underline{r}_i). 
 \end{array}
 \eeq
\end{proposition}
The intuition behind the above theorem is evident from the Lagrangian of the one-shot economic dispatch (\ref{eq:RED}), when $W=T$.   Because TLMP decouples the temporal dependencies of the multi-interval  dispatch,  the optimal dispatch $g_{it}^*$ should always satisfy the individual rationality condition for all $i$ and $t$.

The positive merchandising surplus and (\ref{eq:MS}) are, perhaps, not surprising;  they are  analogous to the same property for LMP when network congestions occur.




==> SufCondiCheckUntruthfulBidIncenUniformP.tex <==
\subsection{{sufficient condition to check untruthfully bidding incentives under rolling-window uniform pricing for storage}} 
\begin{theorem}[{Untruthful bidding incentives under rolling-window uniform pricing}] \label{thm:StorageUntruBidUniformPricingLOC}
There does not exist a uniform pricing scheme under which a price taker storage will bid truthfully over $\Hc$  such that
\ben

\item  storage has $\frac{\partial}{\partial \theta^D_{t} \partial g^D_{t}}f^D_{t} > 0$ and $-\frac{\partial}{\partial \theta^C_{t} \partial g^C_{t}}f^C_{t} > 0$ for bid-in cost curve. 
\item  storage has nonzero LOC under rolling-window dispatch from (\ref{eq:gED}), $\gbf^D(\thetabf^{*})$,$\gbf^C(\thetabf^{*})$, and for all $t$, storage has at least one binding constraint among capacity constraints, ramping constraints and SOC constraints. 
\item  For all $t$, individual optimal dispatch from (\ref{eq:Q}), $\pbf^{D*}$ and $\pbf^{C*}$, has at least one binding constraint among capacity constraints, ramping constraints and SOC constraints.



 \een
\end{theorem}

\textit{Proof\footnote{Some equations works for both charge and discharge so the upscripts, i.e. $D$ for discharge and $C$ for charge, are omitted for simplicity. }:} Because storage has nonzero LOC, we have $\gbf(\thetabf^{*}) \neq \pbf^{*}$.  %$\gbf^D(\thetabf^{D*}) \neq \pbf^{D*}$ and $\gbf^C(\thetabf^{C*}) \neq \pbf^{C*}$.
From conditions  3) of Theorem~\ref{thm:StorageUntruBidUniformPricingLOC}, we know $\psibf^*\bar{\omegabf}^*\underline{\omegabf}^*\bar{\etabf}^*\underline{\etabf}^*\bar{\zetabf}^*\underline{\zetabf}^* \neq \mathbf{0}$. We argue that any infinitesimal change in $f_{t}(\cdot|\theta_{t})$ will not change the optimal solution $\pbf^*_{t}$, \ie   $\frac{\partial}{\partial \theta_{t}} p^{\mbox{\tiny *}}_{t}(\thetabf)=0$. Specifically, suppose that an infinitesimal change of $\theta_{t}^*$ causes a change  $f_{t}(p_{t}^{*}|\theta_{t}) = f_{t}(p_{t}^{*}|\theta_{t})+ \epsilon$.  By the continuity of $f_{t}$ with respect to $\theta_{t}$ and  (\ref{eq:StorageLOCKKT}),  we can always reduce  $-1/\xi^D\psi^{D*}_t+\Delta\eta^{D*}_{(t-1)}-\Delta\eta^{D*}_{t} + \Delta\zeta^{D*}_{t}$ by  $\epsilon$ (or reduce  $-\xi^C\psi^{C*}_t+\Delta\eta^{C*}_{(t-1)}-\Delta\eta^{C*}_{t} + \Delta\zeta^{C*}_{t}$ by  $\epsilon$) so that the KKT condition \eqref{eq:StorageLOCKKT} is still satisfied. Moreover, as long as $\epsilon$ is small enough, all other inequalities in KKT conditions will also hold. Similarly, it can be proved that $\frac{\partial}{\partial \theta_{t}} g_{t}(\thetabf^{*})=0$

%This can also be observed from  \eqref{eq:LOCKKTDerTheta}.
%So we have $\gbf^*_{i}=\nabla f_i^{-1}(\pibf -\Abf^{\intercal}\Delta\etabf^*(\theta_{it}) - \Delta\zetabf^*(\theta_{it}))$. And the optimal value is $\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})-\pibf^{\T}\gbf^*_{i}$.

% Take derivative over $\thetabf_{i}$ on both sides of (\ref{eq:LOCKKT}). We have
% \beq \label{eq:LOCKKTDerTheta}
% \nabla_{\thetabf_{i}}\nabla_{\gbf^*_{i}} f_i(\gbf^*_{i}|\thetabf_{i})+\nabla_{\thetabf_{i}} \gbf^*_{i}\nabla^2_{\gbf^*_{i}} f_i(\gbf^*_{i}|\thetabf_{i}) +\nabla_{\thetabf_{i}}(\Abf^{\intercal}\Delta\etabf^*_{i}) + \nabla_{\thetabf_{i}}(\Delta\zetabf^*_{i}) ={\bf 0},
% \eeq

And the derivative of \eqref{eq:StoragePi_i} over $\theta_{t}$ can be simplified as
\beq \label{eq:StoragePi_i2Derivative}
\begin{array}{l}
 \frac{\partial}{\partial \theta^D_{t}} \Pi(\thetabf) = \frac{\partial}{\partial \theta^D_{t}} f^D_{t}(g^D_{t}(\theta^D_{t})|\theta^D_{t})-\frac{\partial}{\partial \theta^D_{t}} f^D_{t}(p^{D*}_{t} |\theta^D_{t}),\\
  \frac{\partial}{\partial \theta^C_{t}} \Pi(\thetabf) = -\frac{\partial}{\partial \theta^C_{t}} f^C_{t}(g^C_{t}(\theta^C_{t})|\theta^C_{t})+\frac{\partial}{\partial \theta^C_{t}} f^C_{t}(p^{C*}_{t} |\theta^C_{t}),
\end{array}
\eeq

We already know $\gbf^D(\thetabf^{*}) \neq \pbf^{D*}$ and $\frac{\partial}{\partial \theta^D_{t} \partial g^D_{t}}f^D_{t} > 0$. So  $\nabla_{\tiny \thetabf^D} \Pi(\thetabf)  \neq  \mathbf{0}$.
To make more profits, a storage will increase $\theta^D_{t}$ at $t$ when $p^{D*}_{t} < g^{D}_{t}$, and decrease $\theta^D_{t}$ at $t$ when $p^{D*}_{t} > g^{D}_{t}$. Similarly, we can show $\nabla_{\tiny \thetabf^C} \Pi(\thetabf)  \neq  \mathbf{0}$ and corresponding untruthful bidding strategies.

A parallel statement about generators' untruthfully bidding incentives is analyzed in Appendix at Section. \ref{sec:Appendix}.


==> SufConditruthfulBidGenCase.tex <==

\subsection{A toy example to show untruthful bidding incentives under rolling-window LMP} 

Table~I shows the rolling-window economic dispatch and rolling-window prices with window size $W=2$.  The load forecasts $\hat{\dbf}_t=(\hat{d}_{t}, \hat{d}_{t+1})$ are listed and $\hat{d}_{t}=d_t$ being the actual load.  Note that $\hat{\dbf}_t$ contains forecast errors.


%First, the missing money scenario happens in this example. G2 is  underpaid by $\pibf^{\RLMP}_1$ in the interval $t=1$.  Unlike the one-shot LMP case, the underpayment is never compensated under R-LMP. The underpayment is compensated out of the market.   The LOC and MW uplifts to G2 are both $\$250$.

Table I shows the  rolling-window economic dispatch and rolling-window prices when G2 bid true cost \$30/MW, and the dispatch of G2 satisfies the conditions in Theorem~\ref{thm:UntruBidUniformPricingLOC} in Table~I. There is no uniform price can remove LOC uplifts.    For  this example, the argument becomes trivial.  Consider interval $t=1$,  for any price greater than \$25, G1 self-scheduling  would have generated more than $380$ (MW).  If the price is \$25, G2 self-scheduling would have generated zero (MW).

When G2 varied bids from \$30/MW to \$31/MW, it was observed that the dispatch and LMP stayed the same as Table I, and the generation surplus of G2 and LOC were recorded in Table~II.   We observed that, under LMP, when G2 increased its bid above its true marginal cost of generation of \$30/MW, its generation surplus (revenue minus the true cost)  stayed the same while LOC---thus the total profit--- increased. Therefore, G2 had incentive to not to bid truthfully.

\begin{table} [h] \label{tab:rolling}
\begin{psfrags}
\centerline{
\psfrag{gpp1}[c]{\small $(g_{it}^{\RED},\pi_t^{\RLMP},\pi_{it}^{\RTLMP})$}
\psfrag{t=1}[c]{\small $t=1$}
\psfrag{t=2}[c]{\small $t=2$}
\psfrag{t=3}[c]{\small $t=3$}
\psfrag{d}[c]{ $\hat{\dbf}_t$}
\psfrag{g}[c]{\small $\bar{g}_i$}
\psfrag{c}[c]{\small $c_i$}
\psfrag{r}[c]{\small $\underline{r}_i=\bar{r}_i$}
\scalefig{0.5}\epsfbox{figs1/Table1.eps}}
\end{psfrags}
\vspace{-2em}\caption{\small Rolling-window economic dispatch, LMP, and TLMP. Initial generation $\gbf[0]={(370, 50)}$.  Load is settled at the LMP $\pi_t^{\LMP}$ for all $t$.}
\end{table}



\begin{table} [h] \label{tab:Revenue LOC profit}
\begin{psfrags}
\centerline{
\psfrag{gpp1}[c]{\small $(g_{it}^{\RED},\pi_t^{\RLMP},\pi_{it}^{\RTLMP})$}
\psfrag{t=1}[c]{\small $t=1$}
\psfrag{t=2}[c]{\small $t=2$}
\psfrag{t=3}[c]{\small $t=3$}
\psfrag{d}[c]{ $\hat{\dbf}_t$}
\psfrag{g}[c]{\small $\bar{g}_i$}
\psfrag{c}[c]{\small $c_i$}
\psfrag{r}[c]{\small $\underline{r}_i=\bar{r}_i$}
\scalefig{0.3}\epsfbox{figs1/Table2.eps}}
\end{psfrags}
\vspace{-1.5em}\caption{\small Generation surplus, LOC, and profit of G2.}
\end{table}



%
%
%\subsection{\textcolor{blue}{Truthful bidding incentives}}
%
%\tcb{
%We provide a numerical validation of truthful bidding incentives under rolling-window LMP and TLMP. As shown in Theorem~\ref{thm:TLMPBid}, a price taker has incentives to bid truthfully based on its marginal cost of generation.  It is not clear, however, whether a price taker would be truthful under LMP when in the multi-interval rolling-window pricing schemes.  Unlike TLMP, the presence of out-of-the-market uplifts under LMP introduces a new dimension that affect generator's bidding behavior.  The following example shows, indeed, generators under LMP do have incentive to bid above its marginal cost.}
%
%\tcb{
%We considered an example with the same parameter settings as Example II except adding generator G3 with very small market share to serve as a proxy for a price-taking generator.  Table~IV shows the parameter settings, rolling-window economic dispatch and rolling-window prices when G3 bid true cost \$28/MW.  As G3's bid deviated from its marginal cost of 28, the total profit under TLMP did not increase, but the profit under LMP increased.   More importantly, the increase comes precisely from the LOC payment that is computed based on bid rather than the true cost.
%}
%
%\begin{table} [h] \label{tab:Truthful bidding rolling}
%\begin{psfrags}
%\centerline{
%\psfrag{gpp1}[c]{\small $(g_{it}^{\RED},\pi_t^{\RLMP},\pi_{it}^{\RTLMP})$}
%\psfrag{t=1}[c]{\small $t=1$}
%\psfrag{t=2}[c]{\small $t=2$}
%\psfrag{t=3}[c]{\small $t=3$}
%\psfrag{d}[c]{ $\hat{\dbf}_t$}
%\psfrag{g}[c]{\small $\bar{g}_i$}
%\psfrag{c}[c]{\small $c_i$}
%\psfrag{r}[c]{\small $\underline{r}_i=\bar{r}_i$}
%\scalefig{0.5}\epsfbox{figs/Table2.eps}}
%\end{psfrags}
%\vspace{-1em}\caption{\small \textcolor{blue}{Rolling-window economic dispatch, LMP, and TLMP consider price taker G3.}}
%\end{table}
%
%\begin{table} [h] \label{tab:Revenue LOC profit}
%\begin{psfrags}
%\centerline{
%\psfrag{gpp1}[c]{\small $(g_{it}^{\RED},\pi_t^{\RLMP},\pi_{it}^{\RTLMP})$}
%\psfrag{t=1}[c]{\small $t=1$}
%\psfrag{t=2}[c]{\small $t=2$}
%\psfrag{t=3}[c]{\small $t=3$}
%\psfrag{d}[c]{ $\hat{\dbf}_t$}
%\psfrag{g}[c]{\small $\bar{g}_i$}
%\psfrag{c}[c]{\small $c_i$}
%\psfrag{r}[c]{\small $\underline{r}_i=\bar{r}_i$}
%\scalefig{0.35}\epsfbox{figs/Table3.eps}}
%\end{psfrags}
%\vspace{-1.5em}\caption{\small \textcolor{blue}{Profit, LOC and total profit of G3.}}
%\end{table}
%
%






==> ToyExampleRLMPV2.tex <==
\subsection{A toy example to show untruthful bidding incentives under rolling-window LMP} 

As shown in Table~I, generator G3 of small generation capacity to mimic a price taking generator with linear cost function. All assumptions of Theorem~\ref{thm:UntruBidUniformPricingLOC} are fulfilled in this toy example. Table I shows the  rolling-window economic dispatch and rolling-window prices when G3 bid true cost \$28/MW.  When G3 varied bids from \$28/MW to \$29/MW, it was observed that the dispatch and LMP stayed the same as Table IV, and the generation surplus of G3 and LOC were recorded in Table~II.   We observed that, under LMP, when G3 increased its bid above its true marginal cost of generation of \$28/MW, its generation surplus (revenue minus the true cost)  stayed the same while LOC---thus the total profit--- increased. Therefore, G3 had incentive to not to bid truthfully.


\begin{table} [h] \label{tab:Truthful bidding rolling}
\begin{psfrags}
\centerline{
\psfrag{gpp1}[c]{\small $(g_{it}^{\RED},\pi_t^{\RLMP},\pi_{it}^{\RTLMP})$}
\psfrag{t=1}[c]{\small $t=1$}
\psfrag{t=2}[c]{\small $t=2$}
\psfrag{t=3}[c]{\small $t=3$}
\psfrag{d}[c]{ $\hat{\dbf}_t$}
\psfrag{g}[c]{\small $\bar{g}_i$}
\psfrag{c}[c]{\small $c_i$}
\psfrag{r}[c]{\small $\underline{r}_i=\bar{r}_i$}
\scalefig{0.5}\epsfbox{figs1/Table2v2.eps}}
\end{psfrags}
\vspace{-1em}\caption{\small Rolling-window economic dispatch, LMP, and TLMP consider price taker G3. Initial generation  $\gbf[0]={(370, 50, 0)}$. }
\end{table}

\begin{table} [h] \label{tab:Revenue LOC profit}
\begin{psfrags}
\centerline{
\psfrag{gpp1}[c]{\small $(g_{it}^{\RED},\pi_t^{\RLMP},\pi_{it}^{\RTLMP})$}
\psfrag{t=1}[c]{\small $t=1$}
\psfrag{t=2}[c]{\small $t=2$}
\psfrag{t=3}[c]{\small $t=3$}
\psfrag{d}[c]{ $\hat{\dbf}_t$}
\psfrag{g}[c]{\small $\bar{g}_i$}
\psfrag{c}[c]{\small $c_i$}
\psfrag{r}[c]{\small $\underline{r}_i=\bar{r}_i$}
\scalefig{0.3}\epsfbox{figs1/Table3v2.eps}}
\end{psfrags}
\vspace{-1.5em}\caption{\small Generation surplus, LOC, and profit of G3.}
\end{table}



==> UntruthfulBidIncenUniformP.tex <==
\subsection{{Untruthfully bidding incentives under rolling-window uniform pricing for generators}} 

Following theorem points out a scenario in which no uniform pricing schemes can support truthfully bidding incentives.

\begin{theorem}[{Untruthful bidding incentives under rolling-window uniform pricing}] \label{thm:UntruBidUniformPricingLOC}
Let $\{g_{kt}^{\RED}(\thetabf)\}$ be the rolling-window economic dispatch over the entire scheduling horizon $\Hc$ when bid-in cost parameter is $\thetabf$. There does not exist a uniform pricing scheme under which all price-taking generators will bid truthfully, if there exist generators $i$ and  $j$ and interval $t^*  \in \Hc$  such that
\ben

\item generators $i$ and $j$ have different bid-in marginal costs of generation
\[
  \frac{d}{dg} f_{it^*}(g_{it^*}^{\RED}(\thetabf^*))  \ne  \frac{d}{dg} f_{jt^*}(g_{jt^*}^{\RED}(\thetabf^*));
  \]
\item both generators are ``marginal''  in $t^*$, \ie
\[
 g_{it^*}^{\RED}(\thetabf^*) \in (0,\bar{g}_i),~~g_{jt^*}^{\RED}(\thetabf^*) \in (0, \bar{g}_j);
\]
\item and both generators have no binding ramping constraints from intervals $t^*-1$ to $t^*$ and from $t^*$ to $t^*+1$ when bid truthfully.

\item if generators $i$ and $j$ slightly deviate bidding curves in $t^*$, both the rolling-window economic dispatch and individual optimal dispatch will stay the same,\ie $ \frac{\partial}{\partial \theta_{it^*}} g^{\mbox{\tiny \RED}}_{kt}(\thetabf^*)=0,\frac{\partial}{\partial \theta_{jt^*}} g^{\mbox{\tiny \RED}}_{kt}(\thetabf^*)=0,  \frac{\partial}{\partial \theta_{it^*}} g^*_{kt}(\thetabf^*)=0,\frac{\partial}{\partial \theta_{jt^*}} g^*_{kt}(\thetabf^*)=0, \forall k, \forall t \in \Hc$.

\item $\forall k, \forall t \in \Hc,$ generators have $\frac{\partial^2}{\partial \theta_{kt} \partial g_{kt}}f_{kt} > 0$ for bid-in cost (supply) curve.

 \een
\end{theorem}

\textit{Proof:} It's already show in \cite{Guo&Chen&Tong:20arxiv} that, with condition 1), 2) and 3), there does not exist a uniform pricing scheme under which all generators have zero LOC. So the total profit of the generator $i$ is given by
\beq \label{eq:Pi_iGen}
\begin{array}{l}
 \Pi_i(\thetabf) = \pibf^{\T} \gbf^{\RED}_i(\thetabf) - \sum_{t=1}^T q_{it}(g^{\RED}_{it}(\thetabf))\\
+\max_{\gbf_i}\pibf^{\T} \gbf_{i} - \sum_{t=1}^T f_{it}(g_{it}|\theta_{it})\\
- \pibf^{\T} \gbf^{\RED}_i(\thetabf) + \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\thetabf)|\theta_{it}),
\end{array}
\eeq
where, under the price-taker assumption,  the uniform clearing price $\pibf$  is not a function of $\thetabf$. $\{g^{\RED}_{it}(\thetabf)\}$ is the rolling-window economic dispatch over the entire scheduling horizon $\Hc$ under a uniform clearing price $\{\pi_t\}$. The first row of (\ref{eq:Pi_iGen}) is the generation surplus and the lost opportunity cost (LOC) under the bid-in cost curve $\fbf_i(\cdot | \theta_i) = (f_{it}(\cdot |\theta_{it}))$ is represented by the second and third row.

%Let $f_{it}(\cdot|\theta_{it})=\frac{1}{2}\theta_{it}g_{it}^2$. First to solve the optimal value of 
Specifically, The second row of (\ref{eq:Pi_iGen}) follows optimization below:
\beq \label{eq:LOC}
\begin{array}{rll}
&\underset{\gbf_i}{\rm minimize} &  \sum_{t=1}^T f_{it}(g_{it}|\theta_{it})-\pibf^{\T}\gbf_{i}\\
 & {\rm subject~to}&
 (\underline{\etabf}_{i},\bar{\etabf}_{i}):~~ -\underline{\rbf}_i\leq \Abf\gbf_i \leq \bar{\rbf}_i, \\
 & & (\underline{\zetabf}_{i},\bar{\zetabf}_{i}):~~   {\bf 0}\leq \gbf_i \leq\bar{\gbf}_{i}.
\end{array} \hfill
\eeq
By the KKT condition, the optimal solution of the above must satisfy
\beq \label{eq:LOCKKTGen}
\nabla_{\gbf_{i}} f_i(\gbf^*_{i}|\thetabf_{i})-\pibf +\Abf^{\intercal}\Delta\etabf^*_{i} + \Delta\zetabf^*_{i} ={\bf 0},
\eeq
where $\Delta\etabf^*_{i}=\bar{\etabf}^*_{i} - \underline{\etabf}^*_{i}$ and $\Delta\zetabf^*_{i}=\bar{\zetabf}^*_{i} - \underline{\zetabf}^*_{i}$. 


%From conditions 2) and 3) of Theorem~\ref{thm:UntruBidUniformPricingLOC}, we know $(\bar{\eta}^*_{it^*} \underline{\eta}^*_{it^*}\bar{\eta}^*_{i(t^*-1)} \underline{\eta}^*_{i(t^*-1)}\bar{\zeta}^*_{it^*}\underline{\zeta}^*_{it^*})$ $(\bar{\eta}^*_{jt^*} \underline{\eta}^*_{jt^*}\bar{\eta}^*_{j(t^*-1)} \underline{\eta}^*_{j(t^*-1)}\bar{\zeta}^*_{jt^*}\underline{\zeta}^*_{jt^*})\neq 0$. 

%Let $(\bar{\eta}^*_{it^*} \underline{\eta}^*_{it^*}\bar{\eta}^*_{i(t^*-1)} \underline{\eta}^*_{i(t^*-1)}\bar{\zeta}^*_{it^*}\underline{\zeta}^*_{it^*})\neq 0$ 
%Let $\Delta\eta^*_{it}\neq 0$
%and we have $g^*_{it^*} \neq g^{\RED}_{it^*}$. We argue that any infinitesimal change in $f_{it^*}(\cdot|\theta_{it^*})$ will not change the optimal solution $\gbf^*_{i}$, \ie   $\frac{\partial}{\partial \theta_{it^*}} g^{\mbox{\tiny *}}_{it}(\thetabf^*)=0,\forall t$. Specifically, suppose that an infinitesimal change of $\theta_{it^*}^*$ causes a change  $f_{it^*}(g_{it}^{*}|\theta_{it^*}^*) = f_{it^*}(g_{it}^{*}|\theta_{it^*}^*)+ \epsilon$ by the continuity of $f_{it^*}$ with respect to $\theta_{it^*}$,  we can always reduce  $\Delta\eta^*_{i(t^*-1)}-\Delta\eta^*_{it^*} + \Delta\zeta^*_{it^*}$ by  $\epsilon$ so that the KKT condition \eqref{eq:LOCKKTGen} is still satisfied. 

%Moreover, as long as $\epsilon$ is small enough, all other inequalities in KKT conditions will also hold. 

%This can also be observed from  \eqref{eq:LOCKKTDerTheta}.
%So we have $\gbf^*_{i}=\nabla f_i^{-1}(\pibf -\Abf^{\intercal}\Delta\etabf^*(\theta_{it}) - \Delta\zetabf^*(\theta_{it}))$. And the optimal value is $\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})-\pibf^{\T}\gbf^*_{i}$.

% Take derivative over $\thetabf_{i}$ on both sides of (\ref{eq:LOCKKT}). We have
% \beq \label{eq:LOCKKTDerTheta}
% \nabla_{\thetabf_{i}}\nabla_{\gbf^*_{i}} f_i(\gbf^*_{i}|\thetabf_{i})+\nabla_{\thetabf_{i}} \gbf^*_{i}\nabla^2_{\gbf^*_{i}} f_i(\gbf^*_{i}|\thetabf_{i}) +\nabla_{\thetabf_{i}}(\Abf^{\intercal}\Delta\etabf^*_{i}) + \nabla_{\thetabf_{i}}(\Delta\zetabf^*_{i}) ={\bf 0},
% \eeq


So we can rewrite \eqref{eq:Pi_iGen} into 
\beq \label{eq:Pi_i2Gen}
\begin{array}{l}
 \Pi_i(\thetabf^*) = \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\thetabf^*)|\theta_{it})- \sum_{t=1}^T q_{it}(g^{\RED}_{it}(\thetabf^*))\\
+\pibf^{\T}\gbf^*_{i}(\thetabf^*)-\sum_{t=1}^T f_{it}(g^*_{it} (\thetabf^*)|\theta_{it}),
\end{array}
\eeq

And the derivative of \eqref{eq:Pi_i2Gen} over $\theta_{it^*}$ is
% \beq \label{eq:Pi_i2Derivative}
% \begin{array}{l}
%  \frac{\partial}{\partial \theta_{it^*}} \Pi_i(\thetabf^*) = \frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^{\RED}_{it^*}(\thetabf^*)|\theta_{it^*})-\frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^*_{it^*} |\theta_{it^*}),
% \end{array}
% \eeq
\beq \label{eq:Pi_i2Derivative2}
\begin{array}{lcl}
 &\frac{\partial}{\partial \theta_{it^*}} \Pi_i(\thetabf^*) = & \frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^{\RED}_{it^*}(\thetabf^*)|\theta_{it^*})-\frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^*_{it^*} |\theta_{it^*})\\
&& +\sum_{t=1}^T \frac{\partial g^*_{it}}{\partial \theta_{it^*}}(\pi_t-\frac{\partial}{\partial g_{it}} f_{it}(g_{it}^*|\theta_{it}^*))\\
 && = \frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^{\RED}_{it^*}(\thetabf^*)|\theta_{it^*})-\frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^*_{it^*} |\theta_{it^*})\\
 &&+\sum_{t=1}^T \frac{\partial g^*_{it}}{\partial \theta_{it^*}}(\Delta \eta^*_{i(t-1)}-\Delta \eta^*_{it}+\Delta \zeta^*_{it}),
\end{array}
\eeq

We already know $g^*_{it^*} \neq g^{\RED}_{it^*}$ because of nonzero LOC and $\frac{\partial}{\partial \theta_{it} \partial g_{it}}f_{it} > 0$ is given from condition 1). So  $\frac{\partial}{\partial \theta_{it^*}} \Pi_i(\thetabf^*) \neq  0$.
To make more profits, generator $i$ will increase $\theta_{it^*}$ at $t^*$ when $g^*_{it^*} < g^{\RED}_{it^*}$, and decrease $\theta_{it^*}$ at $t^*$ when $g^*_{it^*} > g^{\RED}_{it^*}$.




% \beq \label{eq:Pi_i2Derivative3}
% \begin{array}{l}
%  \frac{\partial}{\partial \theta_{it^*}} \Pi_i(\thetabf^*) = \frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^{\RED}_{it^*}(\thetabf^*)|\theta_{it^*})-\frac{\partial}{\partial \theta_{it^*}} f_{it^*}(g^*_{it^*} |\theta_{it^*})\\
%  +\sum_{t=1}^T \frac{\partial g^*_{it}}{\partial \theta_{it^*}}(\Delta \eta^*_{i(t-1)}-\Delta \eta^*_{it}+\Delta \zeta^*_{it}),
% \end{array}
% \eeq

From \eqref{eq:Pi_i2Derivative2}, if generators bids linear cost function and we have many generators, then $\exists i, \frac{\partial g^*_{it}}{\partial \theta_{it^*}}=0, \forall t$. Linear cost is special because the function $\gbf_i^*(\thetabf_{it^*})$ can be noncontinuous. But for the continuous part, we have
\[
\lim_{d\theta_{it^*} \to 0}\frac{g^*_{it}(\theta_{it*}+d\theta_{it^*})-g^*_{it}(\theta_{it*})}{d\theta_{it^*}}=0, \forall t
\]

%\tcb{Theorem: no uniform price can eliminate the probability that $\frac{\partial}{\partial \theta_{it^*}} g^{\mbox{\tiny *}}_{it}(\thetabf^*)=0,\forall t$, when number of generator is large with linear bidding curves. With figure, easier to state. Objective parallel to constraint or not.}


If bidding curve is nonlinear, mostly $\frac{\partial g^*_{it}}{\partial \theta_{it^*}} \neq 0$.  If $g^*$ has no binding constraints, then it's easy to analyze, but with binding constraints, it's hard to directly judge whether or not $\frac{\partial}{\partial \theta_{it^*}} \Pi_i(\thetabf^*) \neq  0$. However, it's also hard to design a uniform price to have \eqref{eq:Pi_i2Derivative2} for every different generators are 0 as we already know the first two terms are nonzero and the last two terms are nonzero. The only way to get zero in summation is to make the first two terms and the last two terms be inverse to each other.

% From \eqref{eq:LOC}, we also know that $ \sum_{t=1}^T f_{it}(g^*_{it}|\theta_{it})-\pibf^{\T}\gbf^*_{i} \le  \sum_{t=1}^T f_{it}(g^{\RED}_{it}|\theta_{it})-\pibf^{\T}\gbf^{\RED}_{i}$

% to show $\exists \pibf, s.t. $

% \tcr{Further complete}Make asumptions $g^{\RED}$ and $g^*$ both unchange when $\theta$ change. And linear cost function.Then
% \beq \label{eq:toycase}
% \begin{array}{l}
% & \Pi_i(\thetabf_i) = \sum_{t=1}^T f_{it}(g^{\RED}_{it}|\theta_{it})-\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})
% &=\theta_{i}\sum_{t=1}^T(g^{\RED}_{it}-g^*_{it}),\\
% \end{array}
% \eeq
% As $\sum_{t=1}^T(g^{\RED}_{it}-g^*_{it})>0$,$\theta_{i}$ is used for all intervals. $\frac{\partial }{\partial \theta_{i}}\Pi_i(\thetabf_i)=\sum_{t=1}^T(g^{\RED}_{it}-g^*_{it}) >0$.

% \tcr{Further complete}Make asumptions $g^{\RED}$ and $g^*$ both unchange when $\theta$ change and $g^{\RED} 
% \geq g^*$. And $\frac{\partial^2 f_{it}}{\partial \theta_{it} \partial g_{it}}>0$. Then we need to compare only this part $\Pi_i(\thetabf_i) = \sum_{t=1}^T f_{it}(g^{\RED}_{it}|\theta_{it})-\sum_{t=1}^T f_{it}(g^*_{it} |\theta_{it})$.
% \beq \label{eq:Pi_i2Derivative}
% \begin{array}{l}
% & \frac{\partial }{\partial \theta_{ik}}\Pi_i(\thetabf_i) =\sum_{t=1}^T (\frac{\partial }{\partial \theta_{it}}f_{it}(g^{\RED}_{it}|\theta_{it})-\frac{\partial }{\partial \theta_{it}}f_{it}(g^{*}_{it}|\theta_{it})),
% \end{array}
% \eeq

% If the generator bids truthfully with its marginal cost of generation,  $\thetabf=\thetabf^*$ and $f_t(\gbf^{\RED}|\theta_t)= q_t(\gbf^{\RED})$, Eq. \eqref{eq:dsdq} becomes
% \beq
% \frac{\partial}{\partial \theta_k} \Pi (\thetabf^*)= \sum_{t} \frac{\partial}{\partial \theta_k^*} g^{\mbox{\tiny R-ED}}_t(\thetabf)\Delta\rho^*_t = 0, \label{eq:dsdq4}
% \eeq
% % The KKT condition gives
% % \bea \label{eq:KKT}
% % \nabla f_i(\gbf_i^*) - \lambdabf^* + \Abf^{\intercal}\Delta\mubf_i^* + \Delta\rhobf_i^* = {\bf 0}
% % \eea
% % where $\Delta\mubf_i^*=\bar{\mubf}^*_i - \underline{\mubf}^*_i$ and $\Delta\rhobf_i^*=\bar{\rhobf}^*_i - \underline{\rhobf}^*_i$.



% \tcr{Try lower bound analysis, but this may be incorrect}
% We have $\max_{g_{it}}\pibf^{\T} g_{it} - \sum_{t=1}^T f_{it}(g_{it}|\theta_{it}) \geq 0$. Besides, note that $\forall t, g^{\RED}_{it}(\theta_{it})\le \bar{g}_i$, and the bid-in cost (supply) curve is increasing, so $q_{it}(g^{\RED}_{it}(\theta_{it})) \le q_{it}(\bar{g}_i)$, so we have
% \beq 
% \begin{array}{lcl}
% &\Pi_i(\thetabf_i) &\geq - \sum_{t=1}^T q_{it}(g^{\RED}_{it}(\theta_{it})) + \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}) \\
% &&\geq \sum_{t=1}^T f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}) - \sum_{t=1}^T q_{it}(\bar{g}_i)
% \end{array}
% \eeq

% We know that $\sum_{t=1}^T q_{it}(\bar{g}_i)$ is a finite constant, and $\lim_{\theta_i \rightarrow +\infty}  f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it}) \rightarrow +\infty$. So the lower bound

% \tcr{not ok, as max part will influence}Make asumptions like linear cost curve, to have max optimal value is 0 even when $\theta$ change a little bit. \tcr{ attention: $\frac{\partial f_{it}(g^{\RED}_{it}(\theta_{it})|\theta_{it})}{\partial \theta_{ik}}\neq \frac{\partial}{\partial \theta_{ik}} g^{\RED}_{it}\thetabf_{i}) (\frac{\partial}{\partial g}f_{it}(g^{\RED}_{it}|\theta_{it})$, so below is wrong and toy case is an example.}
% \beq \label{eq:Pi_i2Derivative}
% \begin{array}{l}
% & \frac{\partial \Pi_i(\thetabf_i)}{\partial \theta_{ik}} =\sum_{t=1}^T \frac{\partial}{\partial \theta_{ik}} g^{\RED}_{it}(\thetabf_{i}) (\frac{\partial}{\partial g}f_{it}(g^{\RED}_{it}|\theta_{it})- \frac{\partial}{\partial g} q_{it}(g^{\RED}_{it})),
% \end{array}
% \eeq


==> intro.tex <==
We consider the problem of pricing energy storage resource (ESR) participation in the real-time wholesale electricity market, motivated by the increasing penetration of utility-scale electric storage \cite{USESMonitor:20Q3,CAISO_StorageBid:20}. Under FERC Order 841 \cite{FERC_Storage:841,FERC_Storage:841-A}, ESRs must be able to participate in the market clearing process as both buyers and sellers.  Given the inherent inter-temporal constraints of battery operation,  it is essential that a centralized pricing mechanism for ESRs and traditional generators provides the necessary dispatch following incentives. Because it is difficult to audit the true cost of ESR operation, it is highly desirable that the pricing mechanism of ESRs offers some degree of incentive compatibility that ensures ESRs bid truthfully.   

The dispatch-following and the truthful bidding incentives are linked inextricably. A pricing scheme unable to provide dispatch following incentives must provide a separate mechanism to compensate for the lost of opportunity costs (LOC) of the market participants.  Typically, an out-of-the-market uplift is provided based on the realized generation and consumption and the submitted bid-in costs.  The dependency of the uplift payments on  ESRs' bids alters the objectives of ESRs' profit maximization, resulting in incentives for ESRs to bid strategically.  

\subsection{Summary of Contributions}
In this paper, we study the problem of dispatch-following and truthful bidding incentives in the context of pricing ESRs in the real-time market under the rolling-window dispatch and pricing models where uncertainties in future  demands and supplies affect dispatch and pricing decisions. 

The main contribution of this work is twofold.  First, we provide a sufficient condition on the rolling-window dispatch  under which no uniform pricing scheme can provide dispatch-following and truthful-bidding incentives to price-taking ESRs.  The lack of dispatch following incentives implies that out-of-the-market uplifts are necessary, and the lack of truthful-bidding incentives implies that a price-taking ESR has incentives to deviate from its true charge and discharge  costs. 

Second, we consider whether a non-uniform (discriminative) pricing mechanism can provide both dispatch-following and truthful-bidding incentives. Note that it is not surprising that a discriminative pricing mechanism can provide dispatch-following incentives; a trivial example is the pay-as-bid (PAB) pricing.  It is not obvious, however, that a discriminative pricing mechanism can provide both incentives simultaneously.    We show that,  as a generalization of the locational marginal pricing (LMP), the temporal-locational marginal pricing (TLMP) \cite{Guo&Tong:18Allerton, Guo&Chen&Tong:20arxiv,Chen&Guo&Tong:20arxiv} not only provides dispatch following incentives thus eliminating the out-of-the-market uplifts but also truthful-bidding incentives for price taking ESRs.  

\subsection{Related Work} 
Wilson in \cite{Wilson:02E} discussed pricing distortion in rolling-window dispatch caused by forecast error and limited look ahead intervals, which resulted in undervaluation of generators' intertemporal ramping capabilities. Recently, \tcr{Jinye} Mays also realized that ESRs with intertemporal state of charge (SOC) constraints also missed dispatch following incentives caused by such pricing distortion \cite{mays2020missing}. To ensure adequate compensation in order to support dispatch following incentives, LOC as uplift payments was proved to be necessary for all uniform pricing schemes \cite{Guo&Chen&Tong:20arxiv}. 

Although the compensation of LOC can support dispatch following incentives of ESRs and generators, such uplift payments are discriminative and may alter truthfully bidding incentives \cite{Gribik&Hogan&Pope:07, cramton2017ElectricityMarket}. All newly proposed multi-interval uniform pricing schemes, like price-preserving multi-interval pricing (PMP)\cite{hogan2020Multi-intervalPricing}, constraint-preserving multi-interval pricing (CMP) \cite{Hua&etal:19TPS} and Multi-settlement LMP (MLMP) \cite{Zhao&Zheng&Litvinov:19TPS}, can reduce but not eliminate LOC in rolling-window dispatch. Besides, nonlinear pricing which may involve discrimination was suggested in \cite{Gribik&Hogan&Pope:07} to eliminate uplift payments, but it also raise more difficulties to analyze the truthfully bidding incentives. 

As for the truthful-bidding strategies of ESRs, different optimal bidding strategies of ESRs are summarized in \cite{de2019StorageBidNoCost}, but the truthful bidding incentives of ESRs are seldom discussed due to the complexity in quantifying true costs for ESRs. This can be overcame by evaluating true cost of ESRs in charging and discharging with the lifetime degradation \cite{he2020StorageDegradation, chen2019StorageLife}. That way, truthful-bidding incentives of ESRs can be analyzed similar to that of generators. 

LMP in single interval is proved to be compatible to truthful-bidding incentives of price-taking market participants in \cite{Baldick18LMPBidTrue}. But uncertainties in rolling-window dispatch brought inefficiencies to initially optimal energy bids of price takers \cite{richstein2020BidsUncertainty}, which also alter the truthful-bidding incentives under rolling-window LMP (R-LMP). Vickrey-Clark-Groves (VCG) mechanism \cite{Vickrey:16JF}, a discriminative pricing mechanism in electricity market \cite{Xu&Low:17TSG}, was proved to be compatible to truthful-bidding incentives. However, undesirable properties and vulnerabilities in practice were shown under VCG in \cite{Hobbs&Rothkopf&Hyde&ONeill:00JRE, Rothkopf&Teisberg&Kahn:90}. Currently, it's still remaining to be solved to propose a applicable multi-interval pricing to support truthful-bidding incentives under rolling-window optimization. 

By applied TLMP proposed in our previous research \cite{Guo&Tong:18Allerton, Guo&Chen&Tong:20arxiv,Chen&Guo&Tong:20arxiv} to ESRs, although non-uniform, rolling-window TLMP (R-TLMP) shed light on supporting both dispatch following incentives and truthful-bidding incentives for ESRs.

%analysis without charging/discharging cost considered, analyzed in \cite{de2019StorageBidNoCost}, withhold capacity stategic bidding to make more profits



%the bidding here we focus is the quantity-pair bids, widely adopted. Many other bidding definition, quantity bids is not mentioned here.




%The internalization of such LOC based on market expectations would often turn out to be wrong and distort the energy offer curve.


%As for truthfully bidding incentives of ESRs,
%However the truthfully bidding behavior becomes tricky to analyze when the {\em out-of-the-market uplift payments} are applied. discusses qualitatively that the internalisation of start-up and other costs based on market expectations would often turn out to be wrong and distort the energy offer curve.




% Due to the imperfect optimization in rolling-window dispatch which has forecast errors and limited look ahead intervals, Wilson commented that pricing was distorted, resulting in undervaluation of generators' intertemporal ramping capabilities \cite{Wilson:02E}. To ensure adequate compensation in order to support dispatch following incentives, the so-called {\em uplift payments} are paid by operators in an {\em out-of-the-market settlement}, for example, the make-whole settlement used in most operators in the U.S. and the lost-of-opportunity-cost (LOC) settlement implemented in ISO-NE. LOC is discriminative and bring incentive issues, other pricing schemes CMP \cite{Hua&etal:19TPS}, PMP\cite{hogan2020Multi-intervalPricing} and MLMP\cite{Zhao&Zheng&Litvinov:19TPS} try but cannot eliminate. MLMP for storage try. TLMP can eliminate. discriminative unavoidable \cite{Guo&Chen&Tong:20arxiv}.


% Correspondingly, missing dispatch following incentives caused by this pricing distortion were analyzed and some pricing schemes were proposed to reduce pricing distortion and LOC \cite{hogan2020Multi-intervalPricing, Guo&Tong:18Allerton, Guo&Chen&Tong:20arxiv, ,Hogan:16,Hua&etal:19TPS}. 


%Pricing distortion in rolling-window dispatch and corresponding newly proposed pricing schemes reducing LOC for generators with intertemporal ramping constraints are discussed in \cite{Wilson:02E, hogan2020Multi-intervalPricing, Guo&Tong:18Allerton, Guo&Chen&Tong:20arxiv,Hogan:16,Hua&etal:19TPS}. Recently, it's also realized that ESRs with intertemporal state of charge (SOC) constraints also missed dispatch following incentives caused by LOC in such pricing distortion \cite{mays2020missing}. And a multi-interval pricing scheme for ESR, Multi-settlement LMP (MLMP) \cite{Zhao&Zheng&Litvinov:19TPS}, was proposed to reduce although not elimination of LOC.



%To support dispatch following incentives in rolling-window dispatch which has pricing distortion induced by forecast errors and limited look ahead intervals \cite{Wilson:02E}

%Due to the imperfect optimization in rolling-window dispatch which has forecast errors and limited look ahead intervals, Wilson commented that pricing was distorted, resulting in undervaluation of generators' intertemporal ramping capabilities \cite{Wilson:02E}. Correspondingly, missing dispatch following incentives caused by this pricing distortion were analyzed and some pricing schemes were proposed to reduce pricing distortion and LOC \cite{hogan2020Multi-intervalPricing, Guo&Tong:18Allerton, Guo&Chen&Tong:20arxiv, ,Hogan:16,Hua&etal:19TPS}. 


%Review of dispatch following incentives: 

 %To ensure adequate compensation and support dispatch following incentives, the so-called {\em uplift payments} are paid by operators in an {\em out-of-the-market settlement}, for example, the make-whole settlement used in most operators in the U.S. and the lost-of-opportunity-cost (LOC) settlement implemented in ISO-NE. LOC is discriminative and bring incentive issues, other pricing schemes CMP \cite{Hua&etal:19TPS}, PMP\cite{hogan2020Multi-intervalPricing} and MLMP\cite{Zhao&Zheng&Litvinov:19TPS} try but cannot eliminate. MLMP for storage try. TLMP can eliminate. discriminative unavoidable \cite{Guo&Chen&Tong:20arxiv}.




%Power systems nowadays are facing increasing integration of the utility-scale energy storage. Even influenced by Covid-19 pandemic, the second quarter (Q2) of 2020 still witness the strongest Q2 storage deployment 168 MW, of which more than two-thirds are front-of-the-meter utility-scale \cite{USESMonitor:20Q3}. Besides, with current 550 MW grid-connected storage, CAISO is planning to increase the installation to 1,500 MW after 2021 \cite{CAISO_StorageBid:20}. To enable a storage resource to provide services within its capacity, FERC Order 841 \cite{FERC_Storage:841} and Order 841-A  \cite{FERC_Storage:841-A} have been issued since 2018, of which one important task was to ensure that an energy storage resource can be dispatched and can set market clearing prices as both a buyer and a seller. In compliance with this order, different storage participation modes and bidding rules are proposed by different ISOs, where efforts are made to make sure storage bid truthfully when participating in the whole-sale electricity market \cite{CAISO_Storage:20, ISONE_Storage:19, MISO_Storage:19, PJM_Storage:19}.



%In our previous research \cite{Guo&Chen&Tong:20arxiv}: (i) it's shown that there does not exist a uniform pricing scheme under which all generators have zero LOC, the out-of-the-market uplifts; (ii) to eliminate the out-of-market uplift payments, the temporal locational marginal pricing (TLMP) is proposed, which is a non-uniform pricing scheme as a generalization of the locational marginal pricing (LMP).
%ii) examples exist that, under LMP, a price-taking generator has incentives to deviate from truthful bidding to take advantage of LOC. 

%Similarly, for the storage resources, we can show that all uniform pricing mechanisms result in non-zero LOC under mild conditions. And we further make two contributions in this research:





%\item Further show in case study section, Properties of real-time rolling-window optimization basically follow trends above empirically. f TLMP not only hold for generator, but also hold for storages. And we expect intertemporal constraints priced with TLMP can all have those properties hold.

%in one-shot optimization, TLMP can support revenue adequacy for ISO and lower consumer payment with ISO rebate, corresponding to which is lower generator profits. 
 


%, which means discrimination is unavoidable in real-time electricity market with rolling-window dispatch




%


%As in the case of storage, proactive market operators and regulators may be able to identify the most relevant conflicts and continue to develop new participation models that facilitate efficient incorporation of new technologies. At present, however, the ability of resources to express their capabilities and receive compensation for flexibility may be incomplete.\cite{mays2020missing}



%1. out of market discriminative, storage violate dispatch signal;(some reference said the out of market payment has this problem but not obviously proved \cite{cramton2017ElectricityMarket}, here we give a detailed situation in Theorem \ref{thm:UntruBidUniformPricingLOC1})

%2. in market discriminative, storage truthfully bidding as price taker. 

%Who should internalize SOC constraint? In both real-time scheduling and pricing, it's being argued whether intertemporal constraints should be considered by ISO or producers? LOC unavoidable, storage internalize in bids (hard nontrivial); in this manuscript, ISO consider it in pricing.

